The Care Label Concept: A Certification Suite for Trustworthy and Resource-Aware Machine Learning

Machine learning applications have become ubiquitous. This has led to an increased effort of making machine learning trustworthy. Explainable and fair AI have already matured. They address knowledgeable users and application engineers. For those who do not want to invest time into understanding the method or the learned model, we offer care labels: easy to understand at a glance, allowing for method or model comparisons, and, at the same time, scientifically well-based. On one hand, this transforms descriptions as given by, e.g., Fact Sheets or Model Cards, into a form that is well-suited for end-users. On the other hand, care labels are the result of a certification suite that tests whether stated guarantees hold. In this paper, we present two experiments with our certification suite. One shows the care labels for configurations of Markov random fields (MRFs). Based on the underlying theory of MRFs, each choice leads to its specific rating of static properties like, e.g., expressivity and reliability. In addition, the implementation is tested and resource consumption is measured yielding dynamic properties. This two-level procedure is followed by another experiment certifying deep neural network (DNN) models. There, we draw the static properties from the literature on a particular model and data set. At the second level, experiments are generated that deliver measurements of robustness against certain attacks. We illustrate this by ResNet-18 and MobileNetV3 applied to ImageNet.

==> images/Fig2alternative/fig2_alt.tex <==
\newcommand{\mpagesize}{0.48}
\begin{figure}
\centering
    \begin{minipage}[t]{\mpagesize\linewidth}
        \centering
        \includegraphics[width=\linewidth]{images/Fig2alternative/Fig2a_alt.pdf}
    \end{minipage}
    \begin{minipage}[t]{\mpagesize\linewidth}
        \centering
        \includegraphics[width=\linewidth]{images/Fig2alternative/Fig2b_alt.pdf}
    \end{minipage}
        \begin{minipage}[t]{\mpagesize\linewidth}
        \centering
        \includegraphics[width=\linewidth]{images/Fig2alternative/Fig2c_alt.pdf}
    \end{minipage}
    \begin{minipage}[t]{\mpagesize\linewidth}
        \centering
        \includegraphics[width=\linewidth]{images/Fig2alternative/Fig2d_alt.pdf}
    \end{minipage}
    \caption{Comparison for runtime in seconds and memory consumption in MiB between GPU (green square, diamond) and CPU (red circle, triangle) implementations of a \ac{mrf} using a grid graph with increasing number of vertices (x-axis). Between GPU and CPU the runtime for the \ac{jt} algorithm improves slightly due to the parallel GPU implementation. However the improvements in runtime come at the cost of a higher memory consumption offset. However, for \ac{lbp} the overhead caused by copy operations from and to the device incur a net increase in runtime and memory.}
    \label{fig:mrf_results}
\end{figure}

==> images/Fig2alternative/fig2_small.tex <==
\newcommand{\mpagesize}{0.24}
\begin{figure}
\centering
    \begin{minipage}[t]{\mpagesize\linewidth}
        \centering
        \includegraphics[width=\linewidth]{images/Fig2alternative/Fig2a_small.pdf}
    \end{minipage}
    \begin{minipage}[t]{\mpagesize\linewidth}
        \centering
        \includegraphics[width=\linewidth]{images/Fig2alternative/Fig2b_small.pdf}
    \end{minipage}
        \begin{minipage}[t]{\mpagesize\linewidth}
        \centering
        \includegraphics[width=\linewidth]{images/Fig2alternative/Fig2c_small.pdf}
    \end{minipage}
    \begin{minipage}[t]{\mpagesize\linewidth}
        \centering
        \includegraphics[width=\linewidth]{images/Fig2alternative/Fig2d_small.pdf}
    \end{minipage}
    %\caption{Comparison for runtime in seconds and memory consumption in MiB between GPU (green square, diamond) and CPU (red circle, triangle) implementations of a \ac{mrf} using a grid graph with increasing number of vertices (x-axis). Between GPU and CPU the runtime for the \ac{jt} algorithm improves slightly due to the parallel GPU implementation. However the improvements in runtime come at the cost of a higher memory consumption offset. However, for \ac{lbp} the overhead caused by copy operations from and to the device incur a net increase in runtime and memory.}
    \caption{We report memory in MiB and runtime in ms consumption for a \ac{mrf} trained with \texttt{pxpy} on a grid graph with increasing grid size on GPU and CPU.}
    \label{fig:mrf_results}
\end{figure}

==> tables/tab1_inference.tex <==
\begin{table}[]
    \centering
    \resizebox{0.6\textwidth}{!}{%
    \begin{tabular}{c|c|c}
    	\toprule
    	& Junction Tree   & LBP   \\ 
    	\midrule 
    	\midrule
    	Time Complexity &  $\bigO(\dom{X}_{C_{max}}^{w})$ &   $\bigO(I|E|\dom{X}_{max}^2\mathcal{N}_{max})$   \\ 
    	\midrule 
    	Memory Complexity  & $\sum_{C \in \mathcal{C}(JT)} \prod_{v\in C} \dom{X}_v $ & $ 2\cdot \sum_{(s,t) \in E} |\mathcal{X}_s| + |\mathcal{X}_t|$   \\ 
    	\midrule 
    	Exact & Yes~\cite{Lauritzen/Spiegelhalter/88a} & Heuristic~\cite{Murphy/etal/99a}  \\ 
    	\bottomrule 
    \end{tabular} 
    }
    \caption{Guarantees and resource consumption of different inference algorithms}
    \label{tab:inference}
\end{table}
